Survival Dynamical Systems for the Population-level Analysis of Epidemics

Motivated by the classical Susceptible-Infected-Recovered (SIR) epidemic models proposed by Kermack and Mckendrick, we consider a class of stochastic compartmental dynamical systems with a notion of partial ordering among the compartments. We call such systems unidirectional Mass Transfer Models (MTMs). We show that there is a natural way of interpreting a uni-directional MTM as a Survival Dynamical System (SDS) that is described in terms of survival functions instead of population counts. This SDS interpretation allows us to employ tools from survival analysis to address various issues with data collection and statistical inference of unidirectional MTMs. In particular, we propose and numerically validate a statistical inference procedure based on SDS-likelihoods. We use the SIR model as a running example throughout the paper to illustrate the ideas.

==> sections/numerical_tables.tex <==


\begin{luacode*}
-- Differential equation of the SIR
function f(x,y,z)
	local beta = 2
	local gamma = 0.5
	return {-beta*x*y, beta*x*y - gamma*y, gamma*y}
end
-- Code to write PGFplots data as coordinates
function print_SIRWithEulerMethod_S(h,npoints,option)
	-- The initial point (x0,y0,z0)
	local x0 = 1
	local y0 = 0.05
	local z0 = 0.0
	local t0 = 0
	local x = x0
	local y = y0
	local z = z0
	local t = t0
	if option~=[[]] then
		tex.sprint("\\addplot["..option.."] coordinates{")
	else
		tex.sprint("\\addplot coordinates{")
	end
	
	--add increments
	for i=1, npoints do
		m = f(x,y,z)
		x = x + h*m[1]
		y = y + h*m[2]
		z = z + h*m[3]
		t = t+h
        tex.sprint("("..t..","..x..")")
	end
	tex.sprint("}")
end
function print_SIRWithEulerMethod_I(h,npoints,option)
	-- The initial point (x0,y0,z0)
	local x0 = 1
	local y0 = 0.05
	local z0 = 0.0
	local t0 = 0
	local x = x0
	local y = y0
	local z = z0
	local t = t0
	if option~=[[]] then
		tex.sprint("\\addplot["..option.."] coordinates{")
	else
		tex.sprint("\\addplot coordinates{")
	end
	
	--add increments
	for i=1, npoints do
		m = f(x,y,z)
		x = x + h*m[1]
		y = y + h*m[2]
		z = z + h*m[3]
		t = t+h
        tex.sprint("("..t..","..y..")")
	end
	tex.sprint("}")
end
function print_SIRWithEulerMethod_R(h,npoints,option)
	-- The initial point (x0,y0,z0)
	local x0 = 1
	local y0 = 0.05
	local z0 = 0.0
	local t0 = 0
	local x = x0
	local y = y0
	local z = z0
	local t = t0
	if option~=[[]] then
		tex.sprint("\\addplot["..option.."] coordinates{")
	else
		tex.sprint("\\addplot coordinates{")
	end
	
	--add increments
	for i=1, npoints do
		m = f(x,y,z)
		x = x + h*m[1]
		y = y + h*m[2]
		z = z + h*m[3]
		t = t+h
        tex.sprint("("..t..","..z..")")
	end
	tex.sprint("}")
end
\end{luacode*}


\newcommand\addScoordinates[3][]{%
\directlua{print_SIRWithEulerMethod_S(#2,#3,[[#1]])}%
}
\newcommand\addIcoordinates[3][]{%
\directlua{print_SIRWithEulerMethod_I(#2,#3,[[#1]])}%
}
\newcommand\addRcoordinates[3][]{%
\directlua{print_SIRWithEulerMethod_R(#2,#3,[[#1]])}%
}


%        tex.sprint("("..t..","..y..")")
%        tex.sprint("("..t..","..z..")")
